The merging dwarf galaxy UM 448: chemodynamics of the ionized gas from VLT integral field spectroscopy

Using VLT/FLAMES optical IFU observations, we present a detailed study of UM 448, a nearby Blue Compact Galaxy (BCG) previously reported to have an anomalously high N/O abundance ratio. NTT/SuSI2 images reveal a morphology suggestive of a merger of two systems of contrasting colour, whilst our H-alpha emission maps resolve UM 448 into three separate regions that do not coincide with the stellar continuum peaks. UM 448 exhibits complex emission line profiles, with lines consisting of a narrow, central component, an underlying broad component and a third, narrow blue-shifted component. Radial velocity maps show signs of solid body rotation across UM 448, with a projected rotation axis that correlates with the continuum morphology of the galaxy. A spatially-resolved, chemodynamical analysis is presented. Whilst the eastern tail of UM 448 has electron temperatures (Te) that are typical of BCGs, we find a region within the main body of the galaxy where the narrow and broad [O III] 4363 line components trace temperatures differing by 5000K and oxygen abundances differing by 0.4 dex. We measure spatially resolved and integrated ionic and elemental abundances for O, N, S and Ne throughout UM 448, and find they do not agree, possibly due the flux-weighting of Te from the integrated spectrum. This has significant implications for abundances derived from long-slit and integrated spectra of star-forming galaxies in the nearby and distant universe. A region of enhanced N/O ratio is indeed found, extended over a ~0.6 kpc^2 region within the main body of the galaxy. Contrary to previous studies, however, we do not find evidence for a large Wolf-Rayet population, and conclude that WR stars alone cannot be responsible for producing the observed N/O excess. Instead, the location and disturbed morphology of the N-enriched region suggests that interaction-induced inflow of metal-poor gas may be responsible.

==> tables/um448_avg_abund_binned_paper.tex <==
\begin{table}
\begin{center}
\begin{footnotesize}
\title{UM~448: Average SFR ionic and elemental abundances derived from maps.}
\begin{tabular}{|l|c|c|c|}
\hline   
 & \multicolumn{3}{c|}{C1} \\
\cline{2-4}
& SFR1 & SFR2 & SFR 3 \\
\hline   
O$^+/H^+$ $\times10^5$ &       7.45$\pm$      4.01 &       6.88$\pm$      4.61 &       6.66$\pm$      5.34 \\  
O$^{++}/H^+$ $\times10^5$ &       5.66$\pm$      3.68 &       4.06$\pm$      2.08 &       3.89$\pm$      7.09 \\  
O/H $\times10^4$ &       1.29$\pm$      0.60 &       1.09$\pm$      0.59 &       0.84$\pm$      0.95 \\  
12+log(O/H) &       8.05$\pm$      0.25 &       7.99$\pm$      0.20 &       7.61$\pm$      0.63 \\  
Z/\Zsol &       0.25$\pm$      0.12 &       0.21$\pm$      0.12 &       0.16$\pm$      0.19 \\  

N$^+/H^+$ $\times10^6$ &       4.12$\pm$      1.60 &       4.61$\pm$      1.69 &       2.98$\pm$      1.89 \\  
N/H $\times10^6$ &       7.10$\pm$      2.64 &       8.01$\pm$      3.59 &       5.28$\pm$      2.89 \\  
log(N$^+$/O$^+$) &      -1.23$\pm$      0.23 &      -1.13$\pm$      0.37 &      -1.24$\pm$      0.21 \\  

Ne$^{++}/H^+$ $\times10^6$ &       1.74$\pm$      1.39 &       1.96$\pm$      1.71 &       0.97$\pm$      0.98 \\  
Ne/H $\times10^5$ &       4.73$\pm$      5.26 &       6.19$\pm$      6.86 &       3.54$\pm$      6.93 \\  
log(Ne$^{2+}$/O$^{2+}$) &      -0.84$\pm$      0.99 &      -0.63$\pm$      0.92 &      -0.83$\pm$      1.05 \\  

S$^+/H^+$ $\times10^7$ &       8.49$\pm$     10.96 &       9.38$\pm$      7.03 &       8.17$\pm$      7.38 \\  
S/H $\times10^7$ &       7.02$\pm$      2.81 &       9.78$\pm$      7.43 &       9.69$\pm$      8.41 \\  
log(S$^+$/O$^+$) &      -2.03$\pm$      0.34 &      -1.87$\pm$      0.23 &      -1.88$\pm$      0.18 \\  
\hline
\end{tabular}
\caption{PLEASE NOTE:  This table shows the computed average values derived from the abundance maps.  It probably won't be in the final table and currently acts as a guide when comparing the maps and the summed-spectra results.}
\label{tab:um448_avg_map}
\end{footnotesize}
\end{center}
\end{table}

